The elliptic modular surface of level 4 and its reduction modulo 3

The elliptic modular surface of level 4 is a complex K3 surface with Picard number 20. This surface has a model over a number field such that its reduction modulo 3 yields a surface isomorphic to the Fermat quartic surface in characteristic 3, which is supersingular. The specialization induces an embedding of the N\'eron-Severi lattices. Using this embedding, we determine the automorphism group of this K3 surface over a discrete valuation ring of mixed characteristic whose residue field is of characteristic 3. The elliptic modular surface of level 4 has a fixed-point free involution that gives rise to the Enriques surface of type IV in Nikulin-Kondo-Martin's classification of Enriques surfaces with finite automorphism group. We investigate the specialization of this involution to characteristic 3.

==> 2quadrangles.tex <==
\renewcommand{\PStextplot}[3]%
{\rlap{\hskip -85.3727945361pt \hbox{\hskip #1pt%
\raise #2pt \hbox{#3}}}}%%


==> Dquadrangle.tex <==
\renewcommand{\PStextplot}[3]%
{\rlap{\hskip -85.3727945361pt \hbox{\hskip #1pt%
\raise #2pt \hbox{#3}}}}%%


==> IVStar.tex <==
\renewcommand{\PStextplot}[3]%
{\rlap{\hskip -182.12862834368pt \hbox{\hskip #1pt%
\raise #2pt \hbox{#3}}}}%%


==> Petersen.tex <==
\renewcommand{\PStextplot}[3]%
{\rlap{\hskip -182.12862834368pt \hbox{\hskip #1pt%
\raise #2pt \hbox{#3}}}}%%


==> quadrangle.tex <==
\renewcommand{\PStextplot}[3]%
{\rlap{\hskip -85.3727945361pt \hbox{\hskip #1pt%
\raise #2pt \hbox{#3}}}}%%

